Streamlined Framework for Agile Forecasting Model Development towards Efficient Inventory Management

This paper proposes a framework for developing forecasting models by streamlining the connections between core components of the developmental process. The proposed framework enables swift and robust integration of new datasets, experimentation on different algorithms, and selection of the best models. We start with the datasets of different issues and apply pre-processing steps to clean and engineer meaningful representations of time-series data. To identify robust training configurations, we introduce a novel mechanism of multiple cross-validation strategies. We apply different evaluation metrics to find the best-suited models for varying applications. One of the referent applications is our participation in the intelligent forecasting competition held by the United States Agency of International Development (USAID). Finally, we leverage the flexibility of the framework by applying different evaluation metrics to assess the performance of the models in inventory management settings.

==> figures/lstm_k_analysis.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=.99\linewidth]{figures/lstm_k_analysis.png}
%   \caption{\texttt{\textcolor{red}{TODO: Add caption here}}}
\caption{Average MASE of cross-validation strategies computed from the top-k hyper-parameters of LSTM.}
  \label{fig:lstm_k_analysis}
\end{figure}



==> tables/cross_validation_old.tex <==


% % provisional table

\begin{table}[ht!]
    \caption{Comparison between different cross-validation strategies on MAE, RMSE, and MASE.}
    \centering
    % \hspace*{-1.5cm}
    \setlength\tabcolsep{3pt} % default value: 6pt
    \begin{adjustbox}{angle=270}
    %\resizebox{\textwidth}{!}{  
    \resizebox{!}{6.7cm}{
    \begin{tabular}{|c|c|c|cc|cc|cc|cc|}
    \hline
    \multirow{2}{*}{\textbf{Metric}} & \multirow{2}{*}{\textbf{Model}}& \multirow{2}{*}{\textbf{CV}} & \multicolumn{2}{c|}{\textbf{USAID}} & \multicolumn{2}{c|}{\textbf{Dairy}} & \multicolumn{2}{c|}{\textbf{Walmart}} & \multicolumn{2}{c|}{\textbf{Kaggle}} \\ 
                          & & & Valid & Test & Valid & Test & Valid & Test & Valid & Test \\ \hline
                          
    \multirow{6}{*}{MAE} & \multirow{3}{*}{LGBM} & TS       & 10.0137 & 11.5569 & 7161391.4212 & 5558112.9484 & 36.7506 & 23.3956 & \textbf{580.6803} & 597.3639 \\ 
                         &                       & KFold    & 10.0155 & 11.5532 & 7176317.4586 & 5569232.9011 & 37.0932 & 23.2935 & 599.9208 & 590.4484 \\ 
                         &                       & Both     & \textbf{10.0090} & \textbf{11.5453} & \textbf{7144916.8711} & \textbf{5523882.3054} & \textbf{35.9823} & \textbf{22.9050} & 580.8532 & \textbf{584.5203} \\ \cline{2-11}
    & \multirow{3}{*}{LSTM}                      & TS       & 11.9099 & 13.1042 & 7575627.0460 & 6335273.6606 & 35.3424 & 29.0396 & \textbf{670.1644} & 718.4960 \\ 
                        &                        & KFold    & 11.9841 & 12.9916 & 7630230.9805 & 6292791.9902 & 36.1612 & 28.2580 & 683.8753 & 718.8560 \\ 
                        &                        & Both     & \textbf{11.8981} & \textbf{12.9634} & \textbf{7543566.9502} & \textbf{6245108.7595} & \textbf{34.9195} & \textbf{27.8836} & 663.3316 & \textbf{704.3535} \\ \hline
                        
    \multirow{6}{*}{RMSE} & \multirow{3}{*}{LGBM} & TS      & 25.8590 & 25.7781 & 12173256.1831 & \textbf{8775138.2741} & 48.3616 & 31.4533 & 935.4448 & 1104.3685 \\ 
    &  & KFold                                              & 25.8619 & 25.7894 & 12239237.0670 & 8798863.8646 & 48.7591 & 31.3252 & 958.9292 & 1107.6369 \\ 
    &  & Both                                               & \textbf{25.8418} & \textbf{25.7653} & \textbf{12137081.3735} & 8796239.0009 & \textbf{47.3134} & \textbf{30.8546} & \textbf{934.8742} & \textbf{1091.7608} \\ \cline{2-11}
    & \multirow{3}{*}{LSTM} & TS                            & 27.7534 & 27.1240 & 12649744.7485 & 9833431.4633 & 47.2544 & 39.1796 & 1115.3168 & 1277.7806 \\ 
    & & KFold                                               & 27.8442 & 27.1370 & 12756249.1796 & 9785865.5912 & 48.3109 & 38.1464 & 1143.2876 & 1269.3243 \\ 
    &  & Both                                               & \textbf{27.7244} & \textbf{27.0234} & \textbf{12604806.5602} & \textbf{9710357.7425} & \textbf{46.7371} & \textbf{37.5913} & \textbf{1102.3221} & \textbf{1248.0318} \\ \hline
    
    \multirow{6}{*}{MASE} & \multirow{3}{*}{LGBM} & TS      & 0.8574 & 1.1740 & 0.8557 & 0.9421 & 1.4166 & 0.7890 & \textbf{0.9508} & 0.8984 \\ 
    &  & KFold                                              & 0.8598 & 1.1728 & 0.8578 & 0.9509 & 1.4288 & 0.7856 & 1.0075 & 0.8742 \\ 
    &  & Both                                               & \textbf{0.8562} & \textbf{1.1700} & \textbf{0.8545} & \textbf{0.9383} & \textbf{1.3886} & \textbf{0.7734} & 0.9564 & \textbf{0.8670} \\ \cline{2-11}
    & \multirow{3}{*}{LSTM} & TS                            & 1.1960 & 1.3493 & 0.9096 & 1.1425 & 1.3641 & 0.9765 & 1.0700 & 1.1382 \\ 
    &  & KFold                                              & 1.2187 & 1.3087 & 0.9154 & 1.1364 & 1.3960 & 0.9455 & 1.0937 & 1.1415 \\ 
    &  & Both                                               & \textbf{1.1952} & \textbf{1.3030} & \textbf{0.9062} & \textbf{1.1213} & \textbf{1.3475} & \textbf{0.9352} & \textbf{1.0602} & \textbf{1.1196} \\ \hline

    \end{tabular}
    }
    \end{adjustbox}
    \label{tab:cross_validation}
\end{table}


